Hierarchical Transfer Convolutional Neural Networks for Image Classification

In this paper, we address the issue of how to enhance the generalization performance of convolutional neural networks (CNN) in the early learning stage for image classification. This is motivated by real-time applications that require the generalization performance of CNN to be satisfactory within limited training time. In order to achieve this, a novel hierarchical transfer CNN framework is proposed. It consists of a group of shallow CNNs and a cloud CNN, where the shallow CNNs are trained firstly and then the first layers of the trained shallow CNNs are used to initialize the first layer of the cloud CNN. This method will boost the generalization performance of the cloud CNN significantly, especially during the early stage of training. Experiments using CIFAR-10 and ImageNet datasets are performed to examine the proposed method. Results demonstrate the improvement of testing accuracy is 12% on average and as much as 20% for the CIFAR-10 case while 5% testing accuracy improvement for the ImageNet case during the early stage of learning. It is also shown that universal improvements of testing accuracy are obtained across different settings of dropout and number of shallow CNNs.

==> CNNmodel.tex <==

In the field of machine learning, CNN is a type of feed-forward artificial neural network where its structure is formed among artificial neurons inspired by the organization of vision neurons \cite{LeCun2015}. The multi-layer CNN has been mainly applied to solve image and video recognition \cite{NIPS2012_4824, Karpathy2014} problems.

The CNN architecture is formed by a stack of distinct layers that transform the input data into an output volume. The distinct types of layers such as convolution layers and pooling layers shown in Figure \ref{fig:cnn} compose the network structure of CNN model. The convolutional layer is an essential part of multi-layer artificial neuron networks. The layer's parameters consist of a set of learnable filters, which have a small receptive field, but extend through the depth of the input volume. Moreover, it is usual to periodically insert a pooling layer in-between successive convolutional layers. Its function is to progressively reduce the spatial size of the representation for decreasing the amount of parameters and computation in the network and for controlling over-fitting. At the end of the structure of CNN model, neurons are fully connected to all activations in the previous layer. The main difference between the CNN model and traditional machine learning arises from the feature engineering perspective, where, for traditional machine learning algorithms, data scientists put significant efforts to build up hand-craft features based on their experiences while CNN can learn these features automatically. 





\begin{figure}

  \centering

  \includegraphics[width=0.45\textwidth]{./Figure/cnn.pdf}\\

  \caption{Architecture of the CNN model}\label{fig:cnn}

\end{figure}






%\begin{figure*}

%  \centering

%  \includegraphics[width=1.0\textwidth]{./Figure/MLvsDP.pdf}\\

%  \caption{Comparison between CNN model and traditional machine learning}\label{fig:ml}

%\end{figure*}





==> Discussion.tex <==


We propose a CNN based bagging learning approach for forecasting hourly loads on big load data through combining advantages of fine-tuning models and bagging learning. We train CNN forecasting models on big load data sets, enhance these models by fine-tuning them on small data sets, and construct many weak forecasting sub-models. And we assemble these weak sub-models to build a strong forecasting model. Experiential results show that fine-tuning models and assembling models can improve forecasting performance by using existing big load data sets. 

The proposed method, however, contains some deficiencies. Firstly, the proposed model cannot merge such long time-series information such as season time-series information. However, the load consumption might be related to seasons. According to experimental results, prediction performance for April is better that those of other three months. Secondly, the optimal number of sub-models cannot be learned in the bagging learning automatically. In our experiments, this number can affect forecasting results to some extent. Nevertheless, we have to determine the number by experiences only. 
